Personalized Federated Learning with Multiple Known Clusters

We consider the problem of personalized federated learning when there are known cluster structures within users. An intuitive approach would be to regularize the parameters so that users in the same cluster share similar model weights. The distances between the clusters can then be regularized to reflect the similarity between different clusters of users. We develop an algorithm that allows each cluster to communicate independently and derive the convergence results. We study a hierarchical linear model to theoretically demonstrate that our approach outperforms agents learning independently and agents learning a single shared weight. Finally, we demonstrate the advantages of our approach using both simulated and real-world data.

==> submission/discussion.tex <==
\section{Discussion}
We have provided a multi-cluster counterpart to current approaches in personalized federated learning. In particular, we combine existing works in personalized federated learning, applied statistics, and hierarchical models in marketing.
